INDUS: Effective and Efficient Language Models for Scientific Applications

Large language models (LLMs) trained on general domain corpora showed remarkable results on natural language processing (NLP) tasks. However, previous research demonstrated LLMs trained using domain-focused corpora perform better on specialized tasks. Inspired by this insight, we developed INDUS, a comprehensive suite of LLMs tailored for the closely-related domains of Earth science, biology, physics, heliophysics, planetary sciences and astrophysics, and trained using curated scientific corpora drawn from diverse data sources. The suite of models include: (1) an encoder model trained using domain-specific vocabulary and corpora to address NLP tasks, (2) a contrastive-learning based text embedding model trained using a diverse set of datasets to address information retrieval tasks and (3) smaller versions of these models created using knowledge distillation for applications which have latency or resource constraints. We also created three new scientific benchmark datasets, CLIMATE-CHANGE NER (entity-recognition), NASA-QA (extractive QA) and NASA-IR (IR) to accelerate research in these multi-disciplinary fields. We show that our models outperform both general-purpose (RoBERTa) and domain-specific (SCIBERT) encoders on these new tasks as well as existing tasks in the domains of interest. Furthermore, we demonstrate the use of these models in two industrial settings -- as a retrieval model for large-scale vector search applications and in automatic content tagging systems.

==> applications_section_review_snapshot.tex <==
\section{Industrial Applications of \cassiopea{}}

We show various industrial applications of \cassiopea{} models for downstream tasks in the scientific domain.

% The following section detail two of the industrial applications of the \cassbase{} model, showcasing its versatility and domain adaptation for downstream tasks in the scientific domain. 

\subsection{Retrieval and Vector Search}

% \paragraph{Data Retrieval Pipelines for NASA Sciences}
% \paragraph{Information Retrieval for Science}

%Our organization developed an open-source science infrastructure to promote open, collaborative and interdisciplinary research. A crucial element of this infrastructure is to leverage enterprise search solutions (sinqua) to manage and increase visibility over the organization's multifaceted data catalog. One of the capabilities of the system is vector search based document retrieval and extractive answer pipeline that comprised of finetuned versions of \cassiopea{} models. To improve relevance of user's search results and user experience, The domain finetuned IR model \cassretbase was used to encode aboth the documents and user queries to retrieve relevant documents over a vector database. To improve search relevancy, the retrieved documents are ranked using a document re-ranker model fine-tuned from \cassbase{} on the MS-MARCO dataset \cite{bajaj2016ms}. Finally, answers are extracted using extractive QA model.

Our organization developed an open-source science infrastructure to promote open and interdisciplinary research, called Science Discovery Engine (SDE). To manage and increase visibility over the organization's multifaceted data catalog, we developed a document retrieval and extractive QA pipeline using the finetuned \cassiopea{} models. We finetuned \cassretbase{} and used it to encode a corpus into a vector database, in order to retrieve relevant documents given a user query. To improve search relevancy, the retrieved documents are ranked using a document re-ranker model fine-tuned from \cassbase{} on the MS-MARCO dataset \cite{bajaj2016ms}. Finally, answers are extracted using an extractive QA model. 

\begin{table}[t!]
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{c|c|c}
\hline
 & \robertabase{}& \cassbase{} \\
\hline
\textsc{ms-marco} (MRR@5) & 35.9 & \textbf{36.4}\\
\nasaqa{}  (MRR@5)&  31.1 & \textbf{33.2} \\
\hline
\end{tabular}
\end{adjustbox}
\caption{MRR@5 on re-ranking \nasaqa{} and MS-MARCO tasks using rerankers finetuned from different base models.}
\label{tab:reranker}
\end{table}

\begin{table}[t!]
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{c|c|c|c}
\hline
\textbf{Model} & \multicolumn{2}{c|}{\textbf{Document Retrieval Score}} & \textbf{Answer Quality} \\
& MRR@1 & MRR@3 & Avg. Quality Score \\
\hline
\robertabase{} & 0.54 & 0.62 & 0.60 \\
\cassbase{} & \textbf{0.69} & \textbf{0.78} & \textbf{0.88} \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Avg. Document Retrieval and Answer Quality Scores for 26 questions formulated by experts across Astrophysics, Biology \& Physical Science, Earth Science, Heliophysics \& Planetary Science domains.}
\label{tab:applications}
\end{table}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{Vectorsearch Diagram.png}
%     \caption{Application of \cassiopea{} model: The Retriever model \cassretbase and passage-reranker model finetuned from \cassbase used in a knowledge discovery framework to improve relevancy of retrieved results}
%     \label{fig-vs-pipe}
% \end{figure}

First, we evaluate the performance of the standalone re-ranker finetuned from \cassbase{} on the \nasaqa{} and MS-MARCO datasets, and compare it to an identical re-ranker finetuned from \robertabase{} in table \ref{tab:reranker}. Here, we measure MRR@5 of correctly ranking the most relevant paragraph for the given question. While the \cassiopea{}-reranker has comparable performance to the \roberta{}-reranker on the MS-Marco dev set, it significantly outperforms the latter on the EarthQA dataset, alluding to better domain contextualization and adaptation of the INDUS-Base model.

We then evaluated the end-to-end performance of the domain-adapted model over using the generic \roberta{} base model in the aforementioned system. Both systems were queried with a set of questions spanning various thematic areas, and then manually scored by human annotators based on the document relevance and correctness of the extracted answers. 

% A \textbf{Document Retrieval Score} of 1 indicates a relevant document is returned as the first result, 0.5 indicates the relevant document appears within the top 3 (with the top result being somewhat relevant), and 0 indicates no relevant document is returned. An \textbf{Answer Quality Score} of 1 indicates the correct answer is returned within the first three snippets (i.e., chunk from the document), 0.5 indicates that the answer is returned in more than three snippets, and 0 indicates no relevant answer is returned. Table \ref{tab:applications} shows the superior scores when using \cassiopea{} models instead of \roberta, and we provide sample questions and responses from both systems in Appendix \ref{app:indus-applications}. 

For assessing document retrieval quality, we use the \textbf{MRR@1} and \textbf{MRR@3} metric, which computes the average reciprocal rank of the highest ranked document from the system's top-1 and top-3 retrieved documents respectively.  For answer quality, experts mark a \textbf{Answer Quality Score}. A score of 1 indicates the correct answer is returned within the first three snippets (i.e., chunk from the document), 0.5 indicates that the answer is returned in more than three snippets, and 0 indicates no relevant answer is returned. Table \ref{tab:applications} shows the superior scores when using \cassiopea{} models instead of \roberta. We provide sample questions and responses from both systems, and a screenshot of the system in Appendix \ref{app:indus-applications}. 


%Furthermore, we speculate that the significant improvement in scores for the Astrophysics and Planetary Science thematic areas is correlated with their substantial representation due to the inclusion of related documents from ADS, which is the largest contributor to the training corpus for INDUS.


% To evaluate effect of the domain adapted model w.r.t the robustness of the pipeline, two search interfaces were created: one used the finetuned models of the general purpose MiniLM model (the default offering of the tool) and the other tool used domain adapted finetuned versions of \cassbase{}. A human expert queried both the systems with a common set of questions spanning across various  thematic areas. The manual scoring strategy is broadly designed to measure performance of two crucial aspects: the document relevance and correctness of extracted answers. the following are the scores used, along with the scoring rubric:

% \textbf{Document retrieval score:} indicates relevance of the retrieved document, with the following interpretations for score:

% 1.0: A relevant document is returned as the first result.

% 0.5: A somewhat relevant document is returned as the first result, with a fully relevant document appearing within the remainder of the top 3 results.

% 0.0: No relevant document is returned


% \textbf{ Answer Score:} Indicates the correctness of the extracted answers. The scores are assigned with the following criteria:

% 1.0: The correct answer is returned within the first three snippets.

% 0.5: The correct answer is returned in more than three snippets, or the answer is somewhat correct but not as expected.

% 0.0: No relevant answer or snippet is returned.






% \paragraph{Retrieval Augmented Generation for Scientific Chatbots}

% % We use the aforementioned infrastructure as a document store. This store can be subsetting to obtain a filtered set of documents to be used as grounding sources for chatbots. This document retrieval back-end system can be combined with any existing open decoder model such as GPT4 \cite{openai2024gpt4technicalreport}  and llama family of models \cite{touvron2023llama} for answer generation, ensuring that the chatbot's responses remain faithful to the content of the retrieved documents, while also giving attribution to the source of origination.

% The aforementioned retrieval system can be used with a decoder model (such as GPT4 \cite{openai2024gpt4technicalreport} or Llama \cite{touvron2023llama}) for answer generation, ensuring that the chatbot's responses remain faithful to the content of the retrieved documents, while also giving attribution to the source of origination.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\columnwidth, height=7cm]{class-perf.png}
    \caption{F1-Scores of the classes over 1036 samples}
    \label{fig:class-perf}
\end{figure}


\subsection{Content Classification}

% A classification task was recently performed using fine-tuned \cassbase{}, to categorize scientific publications into 21 Applied Research Areas identified from the Global Change Master Directory (GCMD). The model achieved high performance in classifying publications into the specified 20 research areas, demonstrating its effectiveness in understanding and categorizing complex scientific texts. The model was evaluated using metrics like precision, recall, and F1-scores for each class, highlighting its reliability across different research areas. The final evaluation was conducted on 1,000 unseen publications, ensuring the model's generalization ability. These classifications are utilized on a research website to enhance publication and dataset discovery and are integrated into a knowledge graph. 

% Additionally, the organization fine-tuned the Google bert base model with the same dataset and compared the performance with that of the custom fine-tuned model. The results showed that the custom fine-tuned model outperformed the base model across almost all classes, as shown in Figure \ref{fig:class-perf}.

We finetuned \cassbase{} to categorize scientific publications into 21 Applied Research Areas identified from the Global Change Master Directory, using a corpus of records annotated by humans. The model achieved high performance in this task, demonstrating its effectiveness in understanding and categorizing complex scientific texts. These classifications are used on a research website to enhance publication and dataset discovery and are integrated into a knowledge graph. We evaluate the model's performance on 1036 unseen publications, and show that \cassbase{} outperforms finetuned \robertabase{} by 16.05\% in terms of macro average F1 score, as shown in Figure \ref{fig:class-perf}. 



% The model was evaluated using metrics like precision, recall, and F1-scores for each class, highlighting its reliability across different research areas. The final evaluation was conducted on 1,000 unseen publications, ensuring the model's generalization ability. These classifications are utilized on a research website to enhance publication and dataset discovery and are integrated into a knowledge graph. 

% Additionally, the organization fine-tuned the Google bert base model with the same dataset and compared the performance with that of the custom fine-tuned model. The results showed that the custom fine-tuned model outperformed the base model across almost all classes, as shown in Figure \ref{fig:class-perf}.



% We finetune  to create models that can efficiently classify tagging the documents in the knowledge discovery framework according to the type of data (images, documentation, raw data, software, etc) or domain areas. This significantly reduces the amount of manual labor and time required to classify a large volume of data

% \paragraph{Research Area Classification}
% Furthermore, in a recent work, Indus Language Model was used to classify publications into approximately 22 categories representing applied research areas. The science team curated a dataset of approximately 900 abstract-subject pairs to fine-tune the model. 
% Furthermore, \cassbase{} was used to classify publications into approximately 22 categories representing applied research areas, by finetuning the base model on 900 abstract-subject pairs.
